Multi-Modal Pre-Training for Automated Speech Recognition

Traditionally, research in automated speech recognition has focused on local-first encoding of audio representations to predict the spoken phonemes in an utterance. Unfortunately, approaches relying on such hyper-local information tend to be vulnerable to both local-level corruption (such as audio-frame drops, or loud noises) and global-level noise (such as environmental noise, or background noise) that has not been seen during training. In this work, we introduce a novel approach which leverages a self-supervised learning technique based on masked language modeling to compute a global, multi-modal encoding of the environment in which the utterance occurs. We then use a new deep-fusion framework to integrate this global context into a traditional ASR method, and demonstrate that the resulting method can outperform baseline methods by up to 7% on Librispeech; gains on internal datasets range from 6% (on larger models) to 45% (on smaller models).

==> sections/figures/econformer.tex <==

\begin{figure}
\centering
	\includegraphics[width=\linewidth]{sections/figures/EConformer.png}
	\caption{An overview of E-Conformer: our ASR training process and deep-fusion approach. Our audio is fed to the pre-trained and frozen AV-BERT model, in addition to the standard conformer. For the conformer side, we leverage the standard conformer embeddings, however add an additional cross-attention against the environmental embeddings in each block. The RNN-T and joint model loss remain unchanged from \cite{gulati2020conformer}.}
	\label{fig:econformer}
\end{figure}


==> sections/figures/overview.tex <==



==> sections/figures/results.tex <==


%\begin{table}
%\tiny
%
%\vspace{0.7em}
%\begin{tabularx}{\linewidth}{lll}
%	\toprule
%		\textbf{Method} & \textbf{Parameters} & \textbf{Alexa-Base} & \textbf{Alexa-query} & \textbf{Alexa-Rare} \\
%	\midrule
%		Conformer-M (Baseline)					& 79M 	&		x	\\
%		A-BERT + Conformer-M		& 79M 	&  	x	\\
%		A/V-BERT + Conformer-M	& 79M 	&		x	\\
%		Conformer-L							& 122M 	&		x	\\
%%	\midrule
%%		Rare Words 					& Coformer-M (Baseline)					& 79M 	&&		29.13	\\
%%									& Audio-Pretraining 	+ Conformer-M		& 79M 	&&  	23.91	\\
%%									& Audio/Video-Pretraining + Conformer-M	& 79M 	&&		20.02	\\
%%									& Conformer-L							& 122M 	&&		14.05	\\
%%	\midrule
%%		Messaging 					& Coformer-M (Baseline)					& 79M 	&&		32.50	\\
%%									& Audio-Pretraining 	+ Conformer-M		& 79M 	&&  	27.28	\\
%%									& Audio/Video-Pretraining + Conformer-M	& 79M 	&&		22.05	\\
%%									& Conformer-L							& 122M 	&&		11.39	\\
%	\bottomrule
%\end{tabularx}
%\end{table}


